Towards Unifying Anatomy Segmentation: Automated Generation of a Full-body CT Dataset via Knowledge Aggregation and Anatomical Guidelines

In this study, we present a method for generating automated anatomy segmentation datasets using a sequential process that involves nnU-Net-based pseudo-labeling and anatomy-guided pseudo-label refinement. By combining various fragmented knowledge bases, we generate a dataset of whole-body CT scans with $142$ voxel-level labels for 533 volumes providing comprehensive anatomical coverage which experts have approved. Our proposed procedure does not rely on manual annotation during the label aggregation stage. We examine its plausibility and usefulness using three complementary checks: Human expert evaluation which approved the dataset, a Deep Learning usefulness benchmark on the BTCV dataset in which we achieve 85% dice score without using its training dataset, and medical validity checks. This evaluation procedure combines scalable automated checks with labor-intensive high-quality expert checks. Besides the dataset, we release our trained unified anatomical segmentation model capable of predicting $142$ anatomical structures on CT data.

==> table_spacing.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{lccccccc}
    \toprule
    Source & Series & Labels & Label Domain & Spacing & Slices & IoU \\
    \midrule
         Pediatric~\cite{jordan2022pediatric} & $ 359 $ & 29 & Full Body & [$  0.52 \pm 0.11 , 0.52 \pm 0.11 , 1.76 \pm 0.52  $]  & $ 306.6 \pm 245.4 $ & \todo{-}\\
         
         Total Segmentator~\cite{wasserthal2022totalsegmentator} & $ 1024 $ & 104 & Full Body & [$  1.5 \pm 0.0 , 1.5 \pm 0.0 , 1.5 \pm 0.0  $]  & $ 259.0 \pm 130.3 $ & \todo{-} \\

         SegTHOR~\cite{lambert2020segthor} &  $ 60 $ & 4 & Thoracic & [$  1.00 \pm 0.09 , 1.00 \pm 0.09 , 2.39 \pm 0.23  $]  & $ 184.7 \pm 30.35 $ & \todo{-} \\
         
         CT50Abdomen~\cite{ma2021abdomenct} & $ 50 $ & 13 & Abdominal & [$  0.81 \pm 0.07 , 0.81 \pm 0.07 , 2.63 \pm 0.52  $]  & $ 95.88 \pm 9.000 $& \todo{-}\\

         MAL Cervix~\cite{landman2015miccai} & $ 50 $ & 4 & Reproductive & \todo{-}  &  \todo{-} & \todo{-}\\

         Amos~\cite{ji2022amos} & $ 500 $ & 5 & Abdominal & \todo{-}  & \todo{-} & \todo{-}\\
         
         RibSeg~\cite{yang2021ribseg} & $ 490 $ & 1 & Ribs & [$  0.74 \pm 0.07 , 0.74 \pm 0.07 , 1.13 \pm 0.14  $]  & $ 359.5 \pm 59.06 $ & \todo{-}\\

         Verse~\cite{sekuboyina2021verse} & $374$ & 28 & Spine & [$  0.79 \pm 0.23 , 0.79 \pm 0.23 , 1.29 \pm 0.65  $]  & $ 444.8 \pm 348.6 $ & \todo{-}\\
         
         ATM~\cite{zhang2023multi} & $ 500 $ & 1 & Respiratory & \todo{-}  & \todo{-} & \todo{-} \\
         
         PARSE~\cite{kuanquan_wang_2022_6361906} & $ 203 $ & 1 & Vessels & [$  0.67 \pm 0.07 , 0.67 \pm 0.07 , 0.99 \pm 0.01  $]  & $ 301.4 \pm 31.22 $ & \todo{-} \\
         
         Pelvic CT~\cite{liu2021deep} & $ 1184 $ & \todo{-} & Bones & \todo{-}  & \todo{-} & \todo{-} \\
         
        
        
        
         \bottomrule
    \end{tabular}
    \caption{Comparison of considered CT datasets for datasets used for label aggregation regarding size, number of labels, label domain, volume spacing, number of slices and segmentation performance of a nnUNet~\cite{isensee2021nnu} in 5-fold cross validation.}
    \label{tab:ch5_datasets_overview}
\end{table*}
